Retrieve in Style: Unsupervised Facial Feature Transfer and Retrieval

We present Retrieve in Style (RIS), an unsupervised framework for facial feature transfer and retrieval on real images. Recent work shows capabilities of transferring local facial features by capitalizing on the disentanglement property of the StyleGAN latent space. RIS improves existing art on the following: 1) Introducing more effective feature disentanglement to allow for challenging transfers (ie, hair, pose) that were not shown possible in SoTA methods. 2) Eliminating the need for per-image hyperparameter tuning, and for computing a catalog over a large batch of images. 3) Enabling fine-grained face retrieval using disentangled facial features (eg, eyes). To our best knowledge, this is the first work to retrieve face images at this fine level. 4) Demonstrating robust, natural editing on real images. Our qualitative and quantitative analyses show RIS achieves both high-fidelity feature transfers and accurate fine-grained retrievals on real images. We also discuss the responsible applications of RIS.

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/alpha_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/alpha_real_v2_low.pdf}
    \vspace{-12pt}
    \caption{
    {\bf Latent direction:}
    The $\alpha$ variable in RIS controls interpolation between the source and the reference images, showing a smooth transition of mouth (top row), hair (middle row) and pose (bottom row).
    }
    \label{fig:alpha}
    \vspace{-2ex}
\end{figure}


==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/compare_t.tex <==
\begin{figure*}[thb]
    \begin{minipage}{0.31\textwidth}
        \begin{center}
            \includegraphics[width=3.2\textwidth]{figures/compare_real_v2_low.pdf}            
        \end{center}
        \vspace{-34ex}
        \caption{
        {\bf Comparison with EIS \cite{collins2020editing}:}
        {\bf (a, b)} show transfers from Reference 1 to the source image; {\bf (c)(d)} from Reference 2. 
        Our method (RIS) generates visually more accurate and natural results.
        {\em E.g.,} EIS changed the skin tone in (a) and shirt color in (c), while RIS does not. 
        RIS also achieves beard transfer around mouth in (d), even though beard on female faces is rare or absent in training data.
        }
        \label{fig:compare}
    \end{minipage}
\end{figure*}



    
    

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/hair_cluster_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/hair_cluster_crop.jpg}
    \vspace{-16pt}
    \caption{
    {\bf Submembership:}
    Contribution scores $\MM_{k}$ from our method allow meaningful clustering. In this figure, each row is a cluster for $k\!=\!\text{hair}$; images within a row are similar, showing that clustering is effective. Across rows, the images differ, showing that there is real variation in the hair.
    }
    \label{fig:hair_cluster}
\end{figure}





==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/interpolations_t.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/interpolations.pdf}
    \caption{Following Eq.~\ref{eq:interpolation}, we scale $\qq_k$ to allow smooth interpolation between facial feature transfers. RIS is able to produce smooth and realistic transitions between the transfers.}
    \label{fig:interpolation}
\end{figure*}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/intersection_t.tex <==
\begin{figure}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/intersection.pdf}
    \caption{{\bf Intersection Ratio}: 
    This figure shows the intersection ratio ({\bf y-axis}) computed against $K$, the number of clusters ({\bf x-axis}). 
    The common channels shared by all clusters decrease as the number of clusters increase. This means that for the same facial feature, images do not share the same contributing channels, validating the ``submembership'' effect discussed in Sec.~{\color{red}{3.1}} of the main paper.
    }
    \label{fig:intersection}
\end{figure}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/iou_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{figures/iou.png}
    \caption{
    TRSI-IoU measures the extent of overlapping identities between two different feature queries on the same face. 
    Methods that disentangle facial features better are expected with smaller TRSI-IoU (see text). We compare a boxplot of TRSI-IoU for RIS and EIS. 
    RIS shows noticeable improvement in the median (red line) with much smaller interquartile range (boxes).
    This suggests our method better disentangles facial features.
    }
    \label{fig:iou}
\end{figure}


==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/my_transfer_t.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/my_transfer_v5.pdf}
    \vspace{-3ex}
    \caption{
    {\bf Facial feature transfer:}
    Our method performs effective semantic editing on real images by transferring facial features from {\bf (b)} a reference image to {\bf (a)} a source image. 
    Our method transfers spatially coherent features (\ie, eyes, nose, mouth) as well as challenging features hair and pose.
    Note that real image editing is not possible with SoTA EIS~\cite{collins2020editing}.
    }
    \label{fig:my_transfer}
    \vspace{-1.5ex}
\end{figure*}


==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/nn_retrieve_t.tex <==
\begin{figure*}
    \includegraphics[width=1\linewidth]{figures/nn_retrieve_real_v2_low.pdf}
    \vspace{-4ex}
    \caption{
    {\bf Facial feature retrieval:}
    We compare fine-grained retrieval between our method RIS (submembership $\MM_k$) and EIS \cite{collins2020editing} (universal $\MM_k$) on real faces. We show 3 faces each from nearest and furthest retrieval (NR and FR). RIS retrieves semantically similar NRs on all facial features while showing variance on non-matching features. Note EIS retrieves very similar NR on eyes and nose with same query image indicating a lack of feature localization.
    \vspace{-1ex}
    }
    \label{fig:nn_retrieve}
\end{figure*}






==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/pose_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/pose_real_v2_low.pdf}
    \vspace{-19pt}
    \caption{
    {\bf Pose transfer} from {\bf (a)} reference to {\bf (b)} source.
    {\bf (c)} Naively copying style coefficients from the first 4 layers of StyleGAN2~\cite{karras2020analyzing} transfers primarily pose and partially hair (shorter hair on left, flatter hair top), showing their style coefficients are entangled in the early layers. 
    {\bf (d)} Our method matches the pose of the reference image and preserves the hair faithfully from the source.
    }
    \label{fig:pose}
    \vspace{-1.5ex}
\end{figure}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/rebuttal_figure_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/rebuttal_figure.pdf}
    \caption{(a) Pose editing from facing left (+pose) to right (-pose); (b) Pose-hair disentanglement \& transfer; (c) Editing Obama; (d) Retrieving hair (Scarlett Johansson); (e) Editing LSUN-cars.}
    \label{fig:rebuttal_fig}
    \vspace{-2ex}
\end{figure}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/supp1_t.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/supp1_new.jpg}
    \caption{Results of facial feature transfer on generated images.}
    \label{fig:supp1}
\end{figure*}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/figures/supp2_t.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/supp_retrieve.pdf}
    \caption{Results of retrieval on generated images.}
    \label{fig:supp2}
\end{figure*}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/latex/AMS_tbl.tex <==
\begin{table}[]
\centering
\begin{tabular}{lcr}
\toprule
& \multicolumn{2}{c}{\bf Attribute Matching Score (\%)}          \\
                            \multicolumn{1}{l}{{\bf Class}}  & \multicolumn{1}{c}{\bf{Ours}}  & \multicolumn{1}{r}{{\bf EIS}}\\

\midrule
Eyes  & 96.3  & 95.4 \\
Nose  & 100.0 & 100.0 \\
Mouth & 81.1  & 75.8 \\
Hair  & 97.5  & 97.1 \\
\bottomrule
\end{tabular}
\caption{We compare AMS between RIS and EIS to measure retrieval accuracy {\em w.r.t.} a given facial feature using a pretrained attribute classifier. 
RIS outperforms EIS in all classes, with \emph{mouth} retrieval being noticeably better.}
\label{table:AMS_tbl}
\vspace{-1ex}
\end{table}

==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/latex/fid.tex <==
\begin{table}[t]
    \centering
    \begin{minipage}{0.22\textwidth}
        \begin{tabular}{lc}
            \toprule
            {\bf Method} & {\bf FID$_\infty$}  \\ 
            \midrule
            StyleGAN2 \cite{karras2020analyzing} & 2.44 \\
            EIS \cite{collins2020editing} & 3.47 \\
            RIS (ours) & 3.73 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{0.23\textwidth}
        \vspace{-6pt}
        \includegraphics[width=\textwidth]{figures/fid_comparison_v2_low.pdf}
    \end{minipage}
    \vspace{-4pt}
    \caption{
        {\bf Image fidelity comparison:} 
        RIS achieves a comparable FID$_\infty$ compared to EIS and is only slightly worse compared to the base StyleGAN2. The larger FID$_\infty$ can be attributed to our capability of OOD generation, \eg, long-hair males or bald females as in the right image.
    }
    \label{table:fid}
    \vspace{-2ex}
\end{table}





==> [CVPR 2021] Retrieve in Style_ Unsupervised Facial Feature Transfer and Retrieval_arXiv/latex/intro_v3.tex <==
\remove{This paper shows how to disentangle the appearance of different facial features. Our method, Retrieve in Style (RIS) is able to control and edit individual facial features without any annotation of attributes. Detailed evaluation shows RIS ability to disentangle features leads to significant improvements in controlled generation. Furthermore, RIS leads to face image retrieval by feature -- one can search for all faces with the same nose, \etc. Evaluating this task then leads to a procedure evaluates how disentangled the representations are. }


\remove{Fine-grained face image editing and transfer using GANs remains an open-ended problem despite advancements in generating realistic high resolution images. %
Under unconditional settings, it is often hard to interpret or control the outputs of GANs. 
Conditional GANs are naturally more amenable thanks to extra annotations, such as manual labels \cite{bao2018towards,lample2017fader,xiao2018elegant,yin2017towards,choi2018stargan,zhang2018generative}, segmentation masks \cite{gu2019mask,lee2020maskgan}, attribute classifiers \cite{he2019attgan}, rendering models \cite{KowalskiECCV2020,usman2019puppetgan}, \etc. 
However, the degree of meaningful control over the generated images is largely dependent on how detailed the annotations are. 
This presents a challenge for fine-grained face editing, since detailed annotations often require additional computation and are difficult or impossible to acquire in the first place (\eg, the distinctive shape of eyes).}


Recent advancements in Generative Adversarial Networks (GANs) \cite{brock2018large,karras2019style,karras2020analyzing} have shown capabilities to generate realistic high resolution images, particularly for faces.
Under unconditional settings, it is often hard to interpret or control the outputs of GANs. 
Conditional GANs are more naturally amenable for semantic editing.
However, the degree of meaningful control over the output images is largely dependent on how detailed the annotations are. 
This presents a challenge for fine-grained face editing as it is often difficult or impossible to annotate datasets with the degree of detail needed for fine-grained editing.

Existing works on face editing typically leverage additional information to guide conditional generation, such as manual labels \cite{bao2018towards,lample2017fader,xiao2018elegant,yin2017towards,choi2018stargan,zhang2018generative}, segmentation masks \cite{gu2019mask,lee2020maskgan}, attribute classifiers \cite{he2019attgan}, rendering models \cite{KowalskiECCV2020,usman2019puppetgan}, \etc.
However, the additional information requires extra computation and is not always available in practice.
In addition, the fine-grained facial features (\eg, a distinctive shape of eyes) are difficult to describe as labels or features.
As an alternative, unsupervised discovery of latent directions in a pretrained GAN \cite{harkonen2020ganspace,voynov2020unsupervised,shen2020interpreting} allows for finding meaningful latent representations in a computationally efficient way. 
However, such approaches are less effective for fine-grained editing compared to supervised approaches. 

Recently, Editing in Style (EIS)~\cite{collins2020editing} proposed a mostly unsupervised method for facial feature transfer.  
While EIS allows semantic editing of spatially coherent facial features (\eg, eyes, nose and mouth), it requires computing a semantic catalog over the whole dataset and separate hyperparameter tuning for each image.
Such requirements make EIS non-scalable to large datasets as commonly encountered in retrieval domains.
In addition, it remains challenging for EIS to control facial features that are difficult to describe as a spatial map, such as hair and head pose.
More importantly, EIS works only on synthetic images and remains untested on how real images could be manipulated.


In this study, we propose Retrieve in Style (RIS), a simple and efficient unsupervised framework that tackles both fine-grained facial feature transfer and retrieval.
Fig.~\ref{fig:teaser} illustrates the capabilities offered by RIS.
RIS improves EIS in several aspects.
First, we discover the ``submembership'' property in the style space, showing that style channels corresponding to a particular feature (\eg, eyes) are different for every image and thus must be computed individually instead of over the entire dataset.
As the discovered channels are image-specific, RIS achieves more precise face editing for not only spatially coherent facial features (\eg, eyes, nose, mouth) but also challenging ones (\ie, hair, pose).
Second, with the discovered ``submembership'', we show it is possible to eliminate EIS's requirements on per-image semantic catalog and per-image hyperparameter tuning, and offer better scalability to larger problems.
Third, the image-specific representations naturally extend RIS for fine-grained facial feature retrieval that was not shown possible in EIS.
Lastly, we demonstrate that RIS offers editing and retrieval of {\em real images} when combined with GAN inversion methods, while EIS worked with synthetic images.
Although RIS is general and can be applied to a wide range of datasets, this study focuses on faces as there are established conventions on facial parts and its relevance in face retrieval applications (\eg, \cite{megreya2008matching,courtois1981target,bartlett1984typicality,lee2004suspect}).

\noindent
{\bf Our contributions are:}
\begin{compactenum}
    \item RIS improves over EIS based on our finding of ``sub-membership'', obtaining better controllability over facial features that are spatially coherent (eyes, nose, mouth) and incoherent (hair pose), while requiring no hyperparameter tuning.
    
    \item We obtain feature-specific representations (\eg, eyes, nose, mouth, hair), which enable face retrieval by fine-grained features that are difficult to describe or annotate even for humans. 
    To our best knowledge, this is the first work to address the fine-grained retrieval problem without supervision.
    
    \item  We show that RIS generalizes to GAN-inverted images, allowing transfer and retrieval on real images that was not shown possible in earlier studies. 
    Results on CelebA-HQ validates that RIS achieves high-quality retrieval on large, real-world datasets.
\end{compactenum}


==> figures/interpolations_t.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=1\linewidth]{figures/interpolations.pdf}
    \caption{Following Eq.~\ref{eq:interpolation}, we scale $\qq_k$ to allow smooth interpolation between facial feature transfers. RIS is able to produce smooth and realistic transitions between the transfers.}
    \label{fig:interpolation}
\end{figure*}

==> figures/rebuttal_figure_t.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/rebuttal_figure.pdf}
    \caption{(a) Pose editing from facing left (+pose) to right (-pose); (b) Pose-hair disentanglement \& transfer; (c) Editing Obama; (d) Retrieving hair (Scarlett Johansson); (e) Editing LSUN-cars.}
    \label{fig:rebuttal_fig}
    \vspace{-2ex}
\end{figure}
